Spatiotemporal Covariance Neural Networks

Modeling spatiotemporal interactions in multivariate time series is key to their effective processing, but challenging because of their irregular and often unknown structure. Statistical properties of the data provide useful biases to model interdependencies and are leveraged by correlation and covariance-based networks as well as by processing pipelines relying on principal component analysis (PCA). However, PCA and its temporal extensions suffer instabilities in the covariance eigenvectors when the corresponding eigenvalues are close to each other, making their application to dynamic and streaming data settings challenging. To address these issues, we exploit the analogy between PCA and graph convolutional filters to introduce the SpatioTemporal coVariance Neural Network (STVNN), a relational learning model that operates on the sample covariance matrix of the time series and leverages joint spatiotemporal convolutions to model the data. To account for the streaming and non-stationary setting, we consider an online update of the parameters and sample covariance matrix. We prove the STVNN is stable to the uncertainties introduced by these online estimations, thus improving over temporal PCA-based methods. Experimental results corroborate our theoretical findings and show that STVNN is competitive for multivariate time series processing, it adapts to changes in the data distribution, and it is orders of magnitude more stable than online temporal PCA.

==> auxCommands.tex <==
% Auxiliary commands (typically for editing)
%   Fernando Gama fgama@seas.upenn.edu

%%%%%%%%%%%%%%%%%%%%
%%                %%
%%    COLORING    %%
%%                %%
%%%%%%%%%%%%%%%%%%%%

%   Check if the package has already been loaded, if it hasn't load it
\makeatletter
    \@ifpackageloaded{xcolor}{}{\usepackage{xcolor}}
\makeatother
%

\newcommand{\red}   [1] {{\color{red} #1}}
\newcommand{\blue}  [1] {{\color{blue} #1}}
\newcommand{\green} [1] {{\color[rgb]{0.10,0.50,0.10}#1}}
\newcommand{\gray}  [1] {{\color[rgb]{0.80,0.80,0.80}#1}}
\newcommand{\black} [1] {{\color{black} #1}}

%%%%%%%%%%%%%%%%%%%%
%%                %%
%%    STYLING     %%
%%                %%
%%%%%%%%%%%%%%%%%%%%

\makeatletter
    \@ifpackageloaded{needspace}{}{\usepackage{needspace}}
\makeatother

\newcommand{\titledParagraph}[1]{\medskip\noindent {\bf #1}}

%%%%%%%%%%%%%%%%%%%%%
%%                 %%
%%    CITATIONS    %%
%%                 %%
%%%%%%%%%%%%%%%%%%%%%
%% Normally, these acts as placeholders for citations

\newcommand{\citeX}{{\color[RGB]{192, 72, 41}[X?]}} % Just a placeholder
\newcommand{\citeText}[1]{{\color[RGB]{192, 72, 41}[#1]}} % Allows to be
    % more specific on the citation that wants to be added.

%%%%%%%%%%%%%%%%
%%            %%
%%    MATH    %%
%%            %%
%%%%%%%%%%%%%%%%

% Uppercase Greek
\newcommand{\uppercaseGreek}[1]{%
    \begingroup
    \ucmathlist\MakeUppercase{#1}%
    \endgroup
}

\newcommand{\ucmathlist}{%
    \def\alpha{\mathrm{A}}%
    \def\beta{\mathrm{B}}%
    \let\gamma=\Gamma
    \let\delta=\Delta
    \def\epsilon{\mathrm{E}}%
    \def\varepsilon{\mathrm{E}}%
    \def\zeta{\mathrm{Z}}%
    \def\eta{\mathrm{H}}%
    \let\theta=\Theta
    \let\vartheta=\Theta
    \def\iota{\mathrm{I}}%
    \def\kappa{\mathrm{K}}%
    \let\lambda=\Lambda
    \def\mu{\mathrm{M}}%
    \def\nu{\mathrm{N}}%
    \let\xi=\Xi
    \let\pi=\Pi
    \let\varpi=\Pi
    \def\rho{\mathrm{P}}%
    \def\varrho{\mathrm{P}}%
    \let\sigma=\Sigma
    \def\tau{\mathrm{T}}%
    \let\upsilon=\Upsilon
    \let\phi=\Phi
    \let\varphi=\Phi
    \def\chi{\mathrm{X}}%
    \let\psi=\Psi
    \let\omega=\Omega
}

%%%% REQUIRES amsthm PACKAGE %%%%
%   Check if the package has already been loaded, if it hasn't load it
\makeatletter
    \@ifpackageloaded{amsthm}{}{
        \let\proof\relax
        \let\endproof\relax
        \usepackage{amsthm}
    }
\makeatother
%
\theoremstyle{plain}
    \newtheorem{theorem}{Theorem}
    \newtheorem{proposition}[theorem]{Proposition}
    \newtheorem{lemma}[theorem]{Lemma}
    \newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
    \newtheorem{definition}{Definition}
    \newtheorem{remark}{Remark}

%% THIS IS A MACRO TO RENEWTHEOREMS %%
\makeatletter
\def\renewtheorem#1{%
    \expandafter\let\csname#1\endcsname\relax
    \expandafter\let\csname c@#1\endcsname\relax
    \gdef\renewtheorem@envname{#1}
    \renewtheorem@secpar
}
\def\renewtheorem@secpar{\@ifnextchar[{\renewtheorem@numberedlike}{\renewtheorem@nonumberedlike}}
\def\renewtheorem@numberedlike[#1]#2{\newtheorem{\renewtheorem@envname}[#1]{#2}}
\def\renewtheorem@nonumberedlike#1{
    \def\renewtheorem@caption{#1}
    \edef\renewtheorem@nowithin{\noexpand\newtheorem{\renewtheorem@envname}{\renewtheorem@caption}}
    \renewtheorem@thirdpar
}
\def\renewtheorem@thirdpar{\@ifnextchar[{\renewtheorem@within}{\renewtheorem@nowithin}}
\def\renewtheorem@within[#1]{\renewtheorem@nowithin[#1]}
\makeatother
%% END OF MACRO %%

==> standardPackageInclusion.tex <==
%!TEX root = ../00-graphFilters.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%                              MISC UTILITY                              %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\usepackage{ifpdf}
%   \ifCLASSINFOpdf conditional works the same way.
\usepackage{xcolor} % Package to handle colors

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%                                CITATION                                %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{cite} % Cites and compresses citation numbers

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%                            GRAPHICS RELATED                            %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage[pdftex]{graphicx}
\graphicspath{{../figures/}}
\DeclareGraphicsExtensions{.pdf} %,.jpeg,.png}

\usepackage{tikz}       % Requried for TikZ graphics
\usepackage{pgfplots}   % Required for auxTikzDefs.sty inclusion
\pgfplotsset{compat=1.15} % Avoid warnings

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%                                  MATH                                  %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{amsmath}
\interdisplaylinepenalty=2500 % Adjusts line breaking to IEEEtran.cls default
%   IEEEtran contains the IEEEeqnarray family of commands that can be used to
%   generate multiline equations as well as matrices, tables, etc., of high
%   quality.
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{amssymb}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%                           SPECIALIZED LISTS                            %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%   Do not use dedicated algorithm environments like those in 'algorithm.sty'
%   or 'algorithm2e.sty' ('algorithmic' is fine, but either in-text or embedded
%   in figure)
%\usepackage{algorithmic}
%\usepackage{algorithmicx}
\usepackage{algorithm}
\usepackage{algpseudocode}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%                               ALIGNMENT                                %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{array} % Enhances array, tabular environments (strongly encouraged)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%                               SUBFIGURE                                %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage[caption=false,font=footnotesize]{subfig}
%   Correct subfigure package (not use subfigure); caption false is needed to
%   avoid violation of IEEE style (doesn't override caption setup in IEEEtran)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%                                 FLOATS                                 %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{stfloats} % Double column floats placed at the bottom
%   WARNING: It may cause problems with other float packages, since it heavily
%   rewrites the float handling kernel

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%                         PDF, URL AND HYPERLINK                         %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{url} % Handling and breaking URLs
